Women's Perspectives on Harm and Justice after Online Harassment

Social media platforms aspire to create online experiences where users can participate safely and equitably. However, women around the world experience widespread online harassment, including insults, stalking, aggression, threats, and non-consensual sharing of sexual photos. This article describes women's perceptions of harm associated with online harassment and preferred platform responses to that harm. We conducted a survey in 14 geographic regions around the world (N = 3,993), focusing on regions whose perspectives have been insufficiently elevated in social media governance decisions (e.g. Mongolia, Cameroon). {Results show} that, on average, women perceive greater harm associated with online harassment than men, especially for non-consensual image sharing. Women also prefer most platform responses compared to men, especially removing content and banning users; however, women are less favorable towards payment as a response. Addressing global gender-based violence online requires understanding how women experience online harms and how they wish for it to be addressed. This is especially important given that the people who build and govern technology are not typically those who are most likely to experience online harms.

==> extra_text.tex <==

Complex and inherently social behaviors like online harassment cannot be understood separate from the context in which they occurred. While the core experience of online harassment may be largely universal across regions and cultures, how people experience harm may vary by individual, context, and culture. For example, non-consensual sharing of intimate images happens across regions and cultures, and it is an intense invasion of privacy regardless of the target’s location—but for women in Pakistan or Saudi Arabia, an intimate image could bring shame to an entire family, creating additional consequences and intensifying an already acutely harmful experience. Shifting toward a focus on the underlying behaviors that motivate harm, instead of the specific content that embodies it, creates an opportunity for platforms to integrate a more nuanced understanding of individual and cultural norms into their existing policies and procedures. 

Many major social media companies with global reach are headquartered in the Silicon Valley region of California, run by a few executives with outsized power [ref]. 


\subsection{Online Harassment Experiences}
\subsubsection{Austria} 
Gender is currently not considered a significant factor in determining internet access in Austria \cite{reidl2020digitale}. A gender gap in STEM education and work persists which disadvantages people who do not identify as men in their capacity to shape online infrastructures \cite{reidl2020digitale}. In Austria, online harassment is often discussed using the umbrella term “internet hate” (ger. “Hass im Netz”). An early study from 2017 found that about 70\% of participants had seen a hate posting on the internet \cite{institut_fur_strategieanalysen_digitalmonitor_2017}. This result later informed the creation of a national counseling center against internet hate (ger. “Beratungsstelle \#GegenHassImNetz”) \cite{koppelsexualisierte}. Other research \cite{kohout_sexuelle_2018} on online harassment in Austria found that 30\% of young women and 13\% of young men between the ages of 11 and 18 have experienced sexual harassment on the internet. This indicates that young women are affected almost three times as much as men by online harassment. Another later study found one third of female participants had experienced a form of online harassment \cite{weisser_ring_studie_2018}. Issues around gender based violence on the internet have been critiqued for some time in Austria by various groups. For instance, in 2013, the hashtag \#aufschrei (eng. “outcry”) was used in German speaking countries to highlight widespread concerns around sexism \cite{fuchs_metoo_2018}. Later in 2017/18, \#metoo as an international feminist movement, also rose to prominence on German speaking social media sites and was also heavily debated in the media over a prolonged period of time. The actions and stories of various activists, journalists \cite{brodnig2016hass} and politicians \cite{koppelsexualisierte} managed to keep online harassment both an important topic in media and policy debates, culminating in a new law \cite{pk_nationalrat_2020} against online hate that e.g., requires social media platforms to quickly delete illegal hate speech. Still, there is overall only little research in Austria on online harassment \cite{weisser_ring_studie_2018,koppelsexualisierte} and tactics to combat it.

\subsubsection{Cameroon}

\subsubsection{Caribbean countries}
The Caribbean region  is a group of heterogeneous countries with diverse backgrounds in political stature, culture, and economic development. As the region has continued to make consistent strides towards more technological integrations, there has also been an equally consistent pattern with abuses transferring from offline to online spaces. Unfortunately, the rates of abuse disproportionately affect women and members of the LGBTQ+ community. Gender-based violence (GBV) is prevalent and in some cases agitated through the use of ICTs. This was evident in the Bahamas where a gender non-conforming woman was brutally beaten by multiple men while they verbally assulted her with homophobic slurs. The woman can be seen enduring blows to the head with a piece of wood. The video was shared online and some made fun of the victim. 

Movements against gbv, limitations and imbalances in legislative protection, implications for small community and reputation intensified 

\subsubsection{China}

\subsubsection{Colombia}
Colombia has been recognized as a patriarchal society, which has caused women to be victims of gender inequality, discrimination, and sexual harassment (Maldonado Gómez, 2009). In the last two decades, some progress has been made to solve these issues. For example, Archila Mauricio (2014) has found changes in the education field by showing that women in Colombia are less illiterate. This study has also shown that there is an increase of female students in primary, middle, and high school, and surprisingly, the percentage of women graduating from the college is higher than men. Nevertheless, women mostly graduate from careers that are related to home care and social assistance work, such as nursing. The author argues that this is caused by barriers women face to enter into the “male” careers. Therefore, Meza-Martinez found that even though these improvements in education have positively impacted the labor market, the women access to men positions (e.g., STEM) have been limited due to discrimination. She also claims that this discrimination is cause by social prejudices determined by the sexual division of labor and not by the level of education or their work experience as it has been assumed. In addition, this has also caused a considerable gender wage gap in the labor market in Colombia. For instance, Badel and Peña (2010) found that men are always paid more than women due to gender bias. As a result, women move out of the labor market to take care of households’ activities, as the low salary does not cover the cost of babysitters, nurseries, among others (Baquero, et al., 2000).
 
The patriarchal society in Colombia has not only caused issues with regards to gender inequality and discrimination for women but have also caused issues sexual harassment. In Colombia, similar to other Latin countries, the sexual harassment has been categorized into 4 types: light sexual harassment (e.g., conversations or jokes with sexual content, or lewd looks or gestures), moderate sexual harassment (e.g., Calls, letters or invitations with sexual intentions), strong sexual harassment (e.g., groping, holding, cornering), and severe sexual harassment (Both physical and mental pressures to have sexual contact) (Vásquez, 2020). Hence, scholars have found that Colombian women are experiencing different types of sexual harassment in the universities (Piqueras, 2013) (Vásquez, 2020), public transportation (quinones), in the workplace (Vidal & de Jesús, 2016), and in the public spaces (also known as street sexual harassment – acoso sexual callejero) (Gil, 2018). However, little is known about the sexual harassment online, especially in social media sites. Examining this is important as in Colombia women not only have been sexually harassed in different contexts, but also have been victims of femicide (i.e., gender-motivated homicide) (Pasquali, 2021). For instance, in 2020, 630 women were murdered on account of their gender in Colombia (Pasquali, 2021). As a result, Colombian women (and some men) have joined the online movement #NiUnaMenos and #NiUnaMás (#NotOneLess & #NotOneMore) in order to make people reflect on the consequences of gender stereotypes that cause unequal power relations between women and men that result in subordination and violence (ONU, 2017). Another online movement that was very influential last year in social media was through the hashtag #Emberaquémonos. This was in response to the femicide against an indigenous young girl from the Embera group committed by members of the Colombian military. Given this situation, online harassment needs to be examined as the level of violence in Colombia against women is alarming. In addition, it should be taken into consideration as one study found that an online commentary turns into verbal violence against a journalist in Colombia (Barrios, et al., 2019). Thus, the authors conducted a content analysis of 592 tweets with the goal of documenting how threats from a political power holder foster the formation of networks engaging in verbal violence on Twitter. Therefore, they found that press freedom was compromised and that the posts of a legitimate actor can cause an extremely polarized discussion among citizens who took sides, and provoked further threats and accusations. These online threats have become a very serious issue, that one journalist who received even a death threat decided to stay away from his social media sites and reported the issue to the police (El Espectador, 2020). The police then found the person responsible behind the account which was reported and also that the person has made multiple threats to other journalists. For this reason, the person was sentenced to 36 months of prison. Based on this, one could argue that scholars need to explore online sexual harassment as there might a problem that is affecting many women without being properly addressed to help them overcome this issue.

\subsubsection{India}

\subsubsection{Korea}
\cite{cheng2021male}

\subsubsection{Malaysia}

\subsubsection{Mexico}

\subsubsection{Mongolia }
Historically, men were responsible for jobs outside their homes such as herding animals, choosing where to move and women were responsible for jobs inside their homes such as raising their children, producing dairy products, and cooking. With urbanization, this balance that has been a case for hundreds of years was somewhat disturbed.  Women have somewhat equal rights in the decision making and everyday life cycle, so compared to many other Asian countries, it might seem that Mongolian women exercise more rights and equality. Gender based violence, domestic violence and sexual harassment is one of the important gender issues and women are the primary victims in Mongolia. While we see a tendency that families preferring to send their daughters to university than sons and women are receiving more education than men, there is still a wage gap and absence in the executive positions that women hold. The Domestic Violence Law was passed in 2004 after extensive public debate, but there is little evidence that the means to enforce it are in place or that there will be adequate resources—human or financial—to implement it effectively. 

\subsubsection{Pakistan}
Pakistan holds the most significant gender gap in technology, with women 38 percent less likely than men to own a mobile and 49 percent less likely to use mobile internet \cite{rowntree2020mobile}. One of the most considerable barriers to gender-equitable participation in this region is online safety (among other obstacles like affordability and relevance), driven in part by fear of contending with harassment \cite{mariscal2019bridging} and risks to one’s reputation \cite{kovacs2013don}. Qualitative studies in Pakistan show that most women using online spaces face online abuse or cyber-misogyny in the form of cyberstalking, impersonation, personal content leakage, abusive messages, online rape threats, etc. \cite{jamil2020suffering, sambasivan2019they}. Such lived experience of online harassment faced by women leads to apprehensive implications offline in the form of emotional, physical, and reputation harm and coercive romantic involvement. This intersection of online and offline spaces has often had severe, even deadly, consequences at times turning lethal for women in Pakistan. For instance, honor killing has also been reported as a result of extreme abuse that women in Pakistan face online \cite{digitalrightsfoundation}. Qandeel Baloch, a social media icon in Pakistan, received a barrage of abuse and harassment for her bold online persona that eventually resulted in her brother murdering her in the name of honor killing \cite{dawnmurder}. Due to Pakistan’s cultural sensitivity, despite having the built-in functionality on social platforms for reporting online abuse, women in Pakistan face many barriers to report to these platforms. Salient barriers include limited awareness of reporting features, a perception that social media platforms would not understand regional problems, and that such regional issues do not fall under community guidelines of reportable content \cite{sambasivan2019they, schoenebeck2020drawing}. Besides limited reporting on online platforms, women in Pakistan feel hesitant to report to law enforcement agencies due to such organizations’ notorious reputation as abusers themselves, bringing disrepute to women, and having outdated technical knowledge \cite{sambasivan2019they}. As an alternative, women reach out to NGOs working in cyber-harassment to work with the legal system on online abuse cases. However, only a limited number of women reach out to these NGOs due to their poor discovery. Moreover, most women are not aware of the cybercrime laws like the Prevention of Electronic Crimes Act 2016 \cite{humarainternet}.  Therefore, with a perception of irrelevancy, limited discovery, and fear of discrediting family honor, women in Pakistan rely on informal support mechanisms like getting help from friends, or they suffer in silence \cite{jamil2020suffering,sambasivan2019they}. 

\subsubsection{Russia}

\subsubsection{Saudi Arabia}
Saudi Arabia is experiencing massive transformation in regards to gender equity. Within the past decade, the Saudi government has taken drastic measures to halt forms of social and religious extremism that exert control over women \cite{SaudiCleric,SaudiSahwa}. In the legal sense, Saudi Arabia has worked on uplifting the women driving ban \cite{SaudiVision}, abolishing the male guardianship \cite{SaudiWomen1}, and issuing anti-harassment laws that include both online and offline interactions \cite{SaudiWorldBank}. Despite many reforms, the appearance of Saudi women in the media and online (e.g. posting everyday photos) is stigmatized and thought to bring shame to the family or tribe (cite). In January 2021, Qamar, a Saudi woman, was reported to be brutally murdered by her brothers for having a public Snapchat account where she vlogs her daily life (cite). Qamar’s story is not an isolated incident, rather a lineage of the so-called ‘honor killings’ (cite) to restore perceived tribal/familial dignity. Social prejudice aside, online spaces are not designed to consider gendered harms in the Arab world broadly. Western online platforms, popularly used by people in Saudi Arabia (cite), are dominated by hateful and sexist posts that are often unmarked by content moderation practices that center the English language (cite). Albadi et al. show that ‘Arabic Twitter’ is populated with malicious bots \cite{albadi2018they,albadi2018they}. Recognizing that this gendered violence is embedded in cultural, social and technical fabrics, little work has been done to investigate what type of social media affordances may protect Saudi women. In the context of HCI, Abokhodair and Vieweg explore online interactions in the Arabian Gulf, highlighting how Saudi and Qatari people often blocked family members on social media to combat community forms of surveillance and judgment \cite{abokhodair2016privacy}. We extend the very few past work \cite{al2016exploratory, abokhodair2016privacy} to explore the harms and marginalization experienced by Saudis online, particularly as it relates to gendered dynamics. 





\begin{table}[t!]
\resizebox{1\textwidth}{!}{
\begin{tabular}{l l}
jobs &
When jobs are scarce, men should have more rights to a job than women.\\
mother\_works &
When a mother works for pay, the children suffer.\\
health &
All in all, how would you describe your state of health these days? \\
people\_trusted &
\vtop{\hbox{\strut Generally speaking, would you say that most people can be trusted or that you need to be}\hbox{\strut  
 very careful in dealing with people?}} \\
take\_advantage &
Do you think most people would try to take advantage of you if they got a chance, or would they try to be fair?\\
marital\_status &
Are you currently: Married/Living together but not married/Divorced/Separated/Widowed/Single\\
children &
Have you had any children?\\
political &
\vtop{\hbox{\strut In political matters, people talk of "the left" and "the right."}\hbox{\strut  How would you place your views on this scale, generally speaking?}}   \\
trust\_people &
How much do you trust people you meet for the first time?\\
police &
How much confidence do you have in police?\\
courts & How much confidence do you have in the courts?\\
religion &
Do you belong to a religion or religious denomination? If yes, which one? \\
secure &
How secure do you feel these days in your neighborhood?\\ 
science\_tech &
All things considered, would you say that the world is better off, or worse off, because of science and technology?\\
violence &
Indicate whether you think violence against other people is -- Never justifiable:Always justifiable\\
savings &
During the past year, did your family: Save money/Just get by/Spent some savings/Spent savings and borrowed money\\
income &
\vtop{\hbox{\strut Below is an income scale on which 1 indicates the lowest income group and 7 the highest income group.}\hbox{\strut  What group is your household in?}}  
\\
gender &
What is your gender? -- Selected Choice\\
gender\_other &
What is your gender? -- Prefer to self--describe -- Text\\
age &
What is your age?\\
education &
What is the highest educational level that you have attained? -- Selected Choice\\
education\_other &
What is the highest educational level that you have attained? -- Other (write in) -- Text\\
race / nationality &
How would you describe yourself? (Choose one or more from the following:) -- Selected Choice\\
race\_other &
How would you describe yourself? (Choose one or more from the following:) -- Other (please specify) -- Text\\
employment &
What is your employment status? -- Selected Choice\\
employment\_other &
What is your employment status? -- Other (write in) -- Text
\\
\end{tabular}
}
\vspace{5pt}
\caption{Demographic questions included in the survey.}
\label{table:survey-variables}
\end{table}



For four demographic questions (\textit{jobs}, \textit{mother\_works}, \textit{income}, and \textit{political} in Table \ref{table:survey-variables}), there was an extra re-coding process as mistakes during our deployment meant three regions had response scales with different numbers of options. We rescaled options using linear interpolation or by omitting an option in analysis. 
We anticipate this is unlikely to impact the regression results described below. 
% While this impacts our regression results described below, we anticipate it is unlikely to impact our results.  



\begin{figure*}[t!]
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
  {\includegraphics[width=\textwidth]{psych-harm.png}}
   \caption{Perceptions of psychological harm}
  \end{subfigure}
    \vspace{10pt}
  \begin{subfigure}[b]{0.48\textwidth}
  {\includegraphics[width=\textwidth]{sexual-harm.png}
    \caption{Perceptions of sexual harm}
  }
  \end{subfigure}
  \vspace{10pt}
  \begin{subfigure}[b]{0.48\textwidth}{
    \includegraphics[width=\textwidth]{safety-harm.png}
        \caption{Perceptions of harm to personal safety }
  }
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}{
    \includegraphics[width=\textwidth]{reputation-harm.png}
     \caption{Perceptions of harm to family reputation }
  }
  \end{subfigure}
 \caption{Women's perceptions of psychological harm (a), sexual harm (b), harm to personal safety (c), and (d) harm to family reputation  across four harassment scenarios. Five (5) indicates the highest level of perceived harm and one (1) indicates the lowest.}
%  \gabriel{I would maybe explain the scale here also, e.g. 5 indicates max. harm.}}
  \label{fig:women-harm}
\end{figure*}

\subsubsection{Comparing women's perceptions of harm to men's}
\label{gender-difference-harm}






%MODELS


\begin{table}[b!]
\resizebox{1\textwidth}{!}{
\begin{tabular}{l | l r r |  l r r |  l r r | l r r }
 & \textbf{photos\_psych} & & 
 & \textbf{photos\_safety} & & 
 & \textbf{photos\_reputation} & & 
 & \textbf{photos\_sexual} & & \\
 & B(SE) & CI(L) & CI(U) & B(SE) & CI(L) & CI(U) & B(SE) & CI(L) & CI(U) & B(SE) & CI(L) & CI(U)


 \\\midrule
(Intercept)   & 4.12 (0.23)*** &  3.66 & 4.58 
& 3.65 (0.24)*** & 3.18 & 4.12
& 3.97 (0.23)*** & 3.52 & 4.43
& 4.33 (0.23)*** & 3.89 &  4.78 \\ \midrule    
gender:Woman   &     0.39 (0.04)***   &  0.32  &  0.48
&  0.47 (0.04)*** & 0.38 & 0.55
& 0.22 (0.04)*** & 0.14 & 0.31
& 0.29 (0.04)*** & 0.21 & 0.37 \\   
gender:Undisclose   &      0.49  (0.15)**   & 0.19  &  0.79
&0.68 (0.16)*** & 0.37 & 0.99
& 0.08 (0.15) & -0.22 & 0.38
& 0.06 (0.15) & -0.23 & 0.36 \\   
gender:Self-describe    &   -0.14 (0.3)***   & -0.73  &  0.46 
&  0.47 (0.29) & -0.12 & 1.06
& -0.04 (0.29) & -0.62 & 0.53
& -0.41 (0.28) & -0.97 &  0.14 \\\midrule  
jobs       &   -0.14 (0.05)**  & -0.24  &-0.04    
& -0.11 (0.05)* & -0.21 & 0
& -0.06 (0.05) & -0.17 & 0.04
& -0.35 (0.05)***& -0.45 & -0.25\\   
mother\_works   &  -0.05  (0.05)  & -0.15  & 0.04
&  0.09 (0.05) & 0 & 0.18
& -0.02 (0.05) & -0.11 & 0.07
& -0.13 (0.05)** & -0.22 & -0.04 \\   
health    &  -0.02 (0.03) & -0.07 & 0.03
&  0.02 (0.03) & -0.03 & 0.07
& 0.02 (0.03) & -0.03 & 0.07
& -0.01 (0.03)& -0.06 & 0.04 \\   
people\_trusted   & 0.27 (0.05)*** &  0.17 & 0.38   
& 0.34 (0.05)*** & 0.23 & 0.44
& 0.2 (0.05)*** & 0.09 & 0.31
& 0.16 (0.05)** & 0.059 & 0.27 \\   
take\_advantage  &  -0.05 (0.01)**    &  -0.07 & -0.01
&  -0.02 (0.01) & -0.05 & 0.01
& -0.01 (0.01) & -0.04 & 0.02
& -0.02 (0.01) & -0.05 & 0.01 \\   
marital\_status:Unmarried    &   -0.04 (0.05) & -0.14 & 0.06
&  0 (0.05) & -0.1 & 0.1
& -0.13 (0.05)* & -0.23 & -0.03
& 0.08 (0.05) & -0.01 & 0.18\\   
children  &   0 (0.02)  &  -0.04 & 0.04
& 0.03 (0.02) & 0  & 0.07
& 0.03 (0.02) & -0.01 & 0.07
& 0.03 (0.02) & -0.01 & 0.07 \\   
political  &    0.02  (0.02) & -0.01  &  0.06
& 0.01 (0.02) & -0.02 & 0.05
& 0.04 (0.02)* & 0.01 & 0.08
& 0.01 (0.02) & -0.02 & 0.05 \\   
trust\_people  &  0  (0.03)  &  -0.05  &  0.06
& -0.03 (0.03) & -0.09 & 0.02
& -0.01 (0.03) & -0.07 & 0.05
& 0.02 (0.03) & -0.03 & 0.08 \\   
police   &   0.01 (0.03)  & -0.05  &  0.08
& 0.03 (0.03) & -0.03 & 0.09
& 0.02 (0.03) & -0.04 & 0.08
& -0.09 (0.03)** & -0.15 & -0.03\\   
courts   &      0.04 (0.03)  & -0.02  &  0.11
& 0.09 (0.03)** & 0.03 & 0.16
& 0.08 (0.03)* & 0.02 & 0.14
& 0.02 (0.03) & -0.04 & 0.08 \\   
secure   &    -0.08 (0.02)**    & -0.13  &  -0.03
& -0.14 (0.02)*** & -0.19 & -0.09
& -0.06 (0.02)* & -0.11 & -0.01
& 0.01 (0.02) & -0.03 & 0.06 \\   
science\_tech   &    0.05 (0.01)***    & 0.02  &  0.09
& 0.01 (0.01) & -0.01 & 0.05
& -0.01 (0.01) & -0.04 & 0.02
& 0.09 (0.01)*** & 0.06 & 0.12 \\   
violence   &     -0.08 (0.02)***   & -0.12  &  -0.05
& -0.07 (0.02)*** & -0.11 & -0.04
& -0.09 (0.02)*** & -0.13 & -0.06
& -0.06 (0.02)***& -0.09 & -0.02 \\   
savings    &      -0.02 (0.02)   & -0.06  &  0.02
& -0.02 (0.02) & -0.06 & 0.02
& -0.01 (0.02) & -0.05 & 0.03
& 0 (0.02) & -0.04 & 0.04 \\   
income    &      -0.01 (0.02)   & -0.04  &  0.02
&  -0.04 (0.02)** & -0.08 & -0.01
& -0.02 (0.02) & -0.05 & 0.01
& 0 (0.02) & -0.03 & 0.03 \\   
age     &  -0.01 (0)   &  -0.01  & 0 
&  -0.01 (0)*** & -0.01 & 0
& -0.01 (0)*** & -0.01 & 0
& 0 (0) & 0 &  0 \\   
education:Bachelors   &    0.15 (0.05)    & 0.06  &  0.24 
& 0.19 (0.05)*** & 0.1  & 0.29
& 0.17 (0.05)*** & 0.08 & 0.26
& 0.11 (0.04)* & 0.02 &  0.2 \\   
education:Postgrad    &    0.21 (0.06)  & 0.08 &  0.33 
& 0.25 (0.06)*** & 0.12 & 0.38
& 0.2 (0.06)** & 0.07 & 0.32
& 0.05 (0.06) & -0.07 &  0.17 \\   
employed:Non-full time  &  -0.02  (0.04) & -0.12  &  0.06 
& -0.02 (0.04) &  -0.11 & 0.07
& 0.01 (0.04) & -0.07 & 0.1
& -0.04 (0.04) &  -0.12 & 0.05 \\   
religion:Have religion  &   0.09 (0.046)*    & 0  &  0.18  
& 0.23 (0.05)*** & 0.13 & 0.32
& 0.23 (0.05)*** & 0.14 & 0.32
& -0.04 (0.04) & -0.12 & 0.05   \\\midrule
$R^2$  & 0.08 & & 
& 0.12 & & 
&0.06 & & 
&0.06 & &  \\      
      
\end{tabular}
}
\vspace{5px}
\caption{Perceived psychological harm (\textbf{psych}), harm to personal safety (\textbf{safety}), harm to family reputation (\textbf{reputation}), sexual harm (\textbf{sexual}) in \textit{photos} scenario. *p<.05, **p<.01, ***p<.001. B = beta; SE = standard error; CI(L) and CI(L) = confidence
intervals at 2.5\% and 97.5\%. 
}
%Rows where there is statistical significance between men and women participants’ responses are colored in grey.}
\label{table:lr-perception-photos}
\end{table}




\begin{table}[t!]
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|lll|lll|lll}
                                               & \textbf{photos\_removing} &       &       & \textbf{photos\_labeling} &       &       & \textbf{photos\_banning} &       &       \\
                                               & B(SE)            & CI(L) & CI(U) & B(SE)            & CI(L) & CI(U) & B(SE)           & CI(L) & CI(U) \\\midrule
(Intercept)                                    & 4.83 (0.21)***   & 4.42  & 5.23  & 4.16 (0.25)***   & 3.66  & 4.66  & 4.54 (0.23)***  & 4.09  & 5     \\\midrule
gender:Woman                                   & 0.07 (0.04)      & 0     & 0.14  & 0.03 (0.05)      & -0.06 & 0.12  & 0.11 (0.04)**   & 0.03  & 0.19  \\
gender:Undisclose                              & 0.14 (0.14)      & -0.13 & 0.41  & 0.02 (0.17)      & -0.3  & 0.35  & 0.02 (0.15)     & -0.28 & 0.31  \\
gender:Self-describe                           & -0.19 (0.26)     & -0.7  & 0.32  & -0.46 (0.32)     & -1.09 & 0.17  & -0.26 (0.29)    & -0.83 & 0.3   \\\midrule
jobs                                           & -0.44 (0.05)***  & -0.53 & -0.35 & -0.37 (0.06)***  & -0.48 & -0.25 & -0.43 (0.05)*** & -0.54 & -0.33 \\
mother\_works                                  & -0.11 (0.04)**   & -0.2  & -0.03 & -0.08 (0.05)     & -0.18 & 0.02  & -0.1 (0.05)*    & -0.2  & -0.01 \\
health                                         & 0.02 (0.02)      & -0.03 & 0.06  & 0.03 (0.03)      & -0.03 & 0.08  & 0.04 (0.03)     & -0.01 & 0.09  \\
people\_trusted                                & 0.06 (0.05)      & -0.03 & 0.16  & 0.09 (0.06)      & -0.03 & 0.2   & 0.09 (0.05)     & -0.01 & 0.2   \\
take\_advantage                                & -0.05 (0.01)**   & -0.07 & -0.02 & -0.03 (0.02)     & -0.06 & 0.01  & -0.03 (0.02)    & -0.06 & 0     \\
marital\_status:Unmarried                     & 0.07 (0.05)      & -0.02 & 0.16  & 0.12 (0.06)*     & 0.01  & 0.23  & 0.01 (0.05)     & -0.08 & 0.11  \\
children                                       & 0 (0.02)         & -0.03 & 0.04  & 0.01 (0.02)      & -0.03 & 0.05  & -0.01 (0.02)    & -0.05 & 0.02  \\
political                                      & -0.01 (0.02)     & -0.04 & 0.02  & 0.01 (0.02)      & -0.02 & 0.05  & -0.02 (0.02)    & -0.05 & 0.01  \\
trust\_people                                  & 0.06 (0.03)*     & 0.01  & 0.11  & 0.01 (0.03)      & -0.05 & 0.07  & 0 (0.03)        & -0.06 & 0.05  \\
police                                         & -0.04 (0.03)     & -0.1  & 0.01  & -0.05 (0.03)     & -0.12 & 0.01  & -0.04 (0.03)    & -0.11 & 0.02  \\
courts                                         & -0.02 (0.03)     & -0.07 & 0.04  & 0.04 (0.04)      & -0.03 & 0.11  & 0.01 (0.03)     & -0.05 & 0.07  \\
secure                                         & 0.05 (0.02)*     & 0     & 0.09  & 0.06 (0.03)*     & 0.01  & 0.11  & 0.02 (0.03)     & -0.03 & 0.06  \\
science\_tech                                  & 0.04 (0.01)**    & 0.02  & 0.07  & 0.01 (0.02)      & -0.03 & 0.04  & 0.06 (0.02)***  & 0.03  & 0.09  \\
violence                                       & -0.04 (0.02)**   & -0.08 & -0.01 & -0.02 (0.02)     & -0.06 & 0.01  & -0.05 (0.02)**  & -0.08 & -0.02 \\
savings                                        & -0.03 (0.02)     & -0.07 & 0.01  & -0.03 (0.02)     & -0.08 & 0.01  & 0 (0.02)        & -0.04 & 0.04  \\
income                                         & 0 (0.02)         & -0.03 & 0.03  & -0.02 (0.02)     & -0.05 & 0.02  & 0.01 (0.02)     & -0.02 & 0.04  \\
age                                            & 0 (0)*           & 0     & 0.01  & 0.01 (0)*        & 0     & 0.01  & 0.01 (0)**      & 0     & 0.01  \\
education:Bachelors           & 0.13 (0.04)**    & 0.05  & 0.21  & 0.16 (0.05)**    & 0.06  & 0.26  & 0.02 (0.05)     & -0.07 & 0.11  \\
education:Postgrad               & 0.13 (0.06)*     & 0.02  & 0.24  & 0.3 (0.07)***    & 0.16  & 0.43  & 0.01 (0.06)     & -0.12 & 0.13  \\
employment:Non-full time & -0.02 (0.04)     & -0.1  & 0.05  & -0.09 (0.05)     & -0.18 & 0.01  & -0.05 (0.04)    & -0.14 & 0.03  \\
religion:Have religion                         & -0.07 (0.04)     & -0.15 & 0.01  & 0.02 (0.05)      & -0.08 & 0.12  & -0.05 (0.05)    & -0.14 & 0.04  \\\midrule
$R^2$                                             & 0.07             &       &       & 0.03             &       &       & 0.05            &       &      
\end{tabular}

}
\vspace{1px}
\caption{Preferences toward \textit{existing} platform responses in \textit{sexual photos} scenario (removing, labeling, banning). *p<.05, **p<.01, ***p<.001. B = beta; SE = standard error; CI(L) and CI(L) = confidence
intervals at 2.5\% and 97.5\%
}
\vspace{-20px}
%Rows where there is statistical significance between men and women participants’ responses are colored in grey.}
\label{table:women-old-remedy}
\end{table}

\begin{table}[t!]
\resizebox{1\textwidth}{!}{
\vspace{-10px}
\begin{tabular}{l|lll|lll|lll|lll}
 & \textbf{photos\_paying} &  &  & \textbf{photos\_apology} &  &  & \textbf{photos\_revealing} &  &  & \textbf{photos\_rating} &  & \\ 
     & B(SE)          & CI(L) & CI(U) & B(SE)           & CI(L) & CI(U) & B(SE)             & CI(L) & CI(U) & B(SE)           & CI(L) & CI(U) \\\midrule
(Intercept)                                    & 3.97 (0.33)*** & 3.32  & 4.61  & 4.08 (0.3)***   & 3.5   & 4.66  & 3.57 (0.3)***     & 2.99  & 4.15  & 3.94 (0.29)***  & 3.36  & 4.52  \\\midrule
gender:Woman                                   & -0.08 (0.06)   & -0.2  & 0.04  & 0.06 (0.05)     & -0.05 & 0.16  & 0.13 (0.05)*      & 0.03  & 0.23  & 0.14 (0.05)**   & 0.03  & 0.24  \\
gender:Undisclose                              & -0.49 (0.22)*  & -0.91 & -0.07 & 0.04 (0.19)     & -0.34 & 0.42  & -0.02 (0.19)      & -0.4  & 0.36  & 0.3 (0.19)      & -0.08 & 0.68  \\
gender:Self-describe                           & -0.34 (0.41)   & -1.15 & 0.47  & -0.09 (0.37)    & -0.81 & 0.64  & -0.28 (0.37)      & -1.01 & 0.45  & 0.3 (0.37)      & -0.42 & 1.03  \\\midrule
jobs                                           & -0.21 (0.07)** & -0.36 & -0.07 & -0.08 (0.07)    & -0.22 & 0.05  & -0.1 (0.07)       & -0.23 & 0.04  & -0.25 (0.07)*** & -0.38 & -0.12 \\
mother\_works                                  & -0.06 (0.07)   & -0.2  & 0.07  & -0.1 (0.06)     & -0.22 & 0.02  & -0.06 (0.06)      & -0.18 & 0.06  & 0 (0.06)        & -0.11 & 0.12  \\
health                                         & 0.06 (0.04)    & -0.01 & 0.14  & 0.02 (0.03)     & -0.04 & 0.09  & 0.11 (0.03)**     & 0.04  & 0.18  & 0.11 (0.03)**   & 0.04  & 0.17  \\
people\_trusted                                & 0.07 (0.08)    & -0.08 & 0.22  & 0.13 (0.07)     & -0.01 & 0.26  & 0.19 (0.07)**     & 0.05  & 0.32  & 0.04 (0.07)     & -0.1  & 0.17  \\
take\_advantage                                & -0.03 (0.02)   & -0.07 & 0.02  & 0 (0.02)        & -0.04 & 0.04  & -0.02 (0.02)      & -0.06 & 0.02  & -0.02 (0.02)    & -0.06 & 0.02  \\
marital\_status:Unmarried                    & 0 (0.07)       & -0.14 & 0.14  & -0.01 (0.06)    & -0.14 & 0.12  & -0.09 (0.06)      & -0.21 & 0.04  & 0.03 (0.06)     & -0.1  & 0.16  \\
children                                       & 0.04 (0.03)    & -0.02 & 0.09  & -0.01 (0.02)    & -0.06 & 0.03  & 0.01 (0.02)       & -0.04 & 0.06  & 0.05 (0.02)*    & 0.01  & 0.1   \\
political                                      & -0.02 (0.02)   & -0.07 & 0.02  & 0 (0.02)        & -0.04 & 0.05  & 0.04 (0.02)       & -0.01 & 0.08  & 0 (0.02)        & -0.04 & 0.04  \\
trust\_people                                  & 0.03 (0.04)    & -0.05 & 0.11  & -0.07 (0.04)    & -0.14 & 0.01  & -0.05 (0.04)      & -0.12 & 0.03  & 0.04 (0.04)     & -0.03 & 0.11  \\
police                                         & -0.08 (0.04)   & -0.16 & 0.01  & -0.05 (0.04)    & -0.12 & 0.03  & -0.07 (0.04)      & -0.15 & 0.01  & -0.06 (0.04)    & -0.14 & 0.02  \\
courts                                         & -0.12 (0.05)** & -0.21 & -0.03 & 0.03 (0.04)     & -0.05 & 0.1   & -0.01 (0.04)      & -0.09 & 0.07  & 0.01 (0.04)     & -0.07 & 0.09  \\
secure                                         & -0.11 (0.04)** & -0.19 & -0.04 & 0.02 (0.03)     & -0.05 & 0.08  & -0.01 (0.03)      & -0.07 & 0.05  & -0.06 (0.03)    & -0.12 & 0     \\
science\_tech                                  & -0.01 (0.02)   & -0.05 & 0.03  & -0.05 (0.02)*   & -0.09 & -0.01 & 0 (0.02)          & -0.04 & 0.04  & -0.01 (0.02)    & -0.05 & 0.03  \\
violence                                       & 0.09 (0.02)*** & 0.04  & 0.14  & -0.03 (0.02)    & -0.08 & 0.01  & 0.01 (0.02)       & -0.03 & 0.05  & -0.04 (0.02)    & -0.09 & 0     \\
savings                                        & 0 (0.03)       & -0.06 & 0.06  & -0.07 (0.03)*   & -0.12 & -0.01 & -0.02 (0.03)      & -0.07 & 0.04  & 0 (0.03)        & -0.06 & 0.05  \\
income                                         & 0.02 (0.02)    & -0.03 & 0.07  & -0.04 (0.02)    & -0.08 & 0     & -0.05 (0.02)*     & -0.09 & -0.01 & 0 (0.02)        & -0.04 & 0.04  \\
age                                            & 0.01 (0)***    & 0     & 0.02  & 0.01 (0)**      & 0     & 0.01  & 0 (0)             & 0     & 0.01  & 0 (0)           & 0     & 0.01  \\
education:Bachelors                    & -0.15 (0.07)*  & -0.28 & -0.03 & 0.06 (0.06)     & -0.06 & 0.17  & 0.06 (0.06)       & -0.06 & 0.17  & -0.05 (0.06)    & -0.16 & 0.07  \\
education:Postgrad               & -0.2 (0.09)*   & -0.38 & -0.02 & 0.36 (0.08)***  & 0.2   & 0.51  & 0.23 (0.08)**     & 0.07  & 0.39  & 0.07 (0.08)     & -0.09 & 0.23  \\
employed:Non-full time  & -0.15 (0.06)*  & -0.27 & -0.03 & -0.05 (0.06)    & -0.16 & 0.06  & -0.06 (0.06)      & -0.17 & 0.05  & -0.11 (0.06)*   & -0.22 & 0     \\
religion:Have religion                         & -0.13 (0.06)*  & -0.26 & 0     & 0.11 (0.06)     & -0.01 & 0.22  & -0.02 (0.06)      & -0.13 & 0.1   & 0.06 (0.06)     & -0.05 & 0.17  \\\midrule
$R^2$                                             & 0.04           &       &       & 0.02            &       &       & 0.02              &       &       & 0.02            &       &      
\end{tabular}

}
\vspace{1px}
\caption{Preferences toward \textit{non-existing} platform responses in \textit{sexual photos} scenario (paying, apology, revealing, rating). *p<.05, **p<.01, ***p<.001. B = beta; SE = standard error; CI(L) and CI(L) = confidence
intervals at 2.5\% and 97.5\%
}
%Rows where there is statistical significance between men and women participants’ responses are colored in grey.}
\label{table:women-new-remedy}
\end{table}




